Mosquito Detection with Neural Networks: The Buzz of Deep Learning

Many real-world time-series analysis problems are characterised by scarce data. Solutions typically rely on hand-crafted features extracted from the time or frequency domain allied with classification or regression engines which condition on this (often low-dimensional) feature vector. The huge advances enjoyed by many application domains in recent years have been fuelled by the use of deep learning architectures trained on large data sets. This paper presents an application of deep learning for acoustic event detection in a challenging, data-scarce, real-world problem. Our candidate challenge is to accurately detect the presence of a mosquito from its acoustic signature. We develop convolutional neural networks (CNNs) operating on wavelet transformations of audio recordings. Furthermore, we interrogate the network's predictive power by visualising statistics of network-excitatory samples. These visualisations offer a deep insight into the relative informativeness of components in the detection problem. We include comparisons with conventional classifiers, conditioned on both hand-tuned and generic features, to stress the strength of automatic deep feature learning. Detection is achieved with performance metrics significantly surpassing those of existing algorithmic methods, as well as marginally exceeding those attained by individual human experts.

==> Images/mlp.tex <==
%% Simple MLP diagram %%

\begin{figure}
\begin{center}
\begin{tikzpicture}
[   cnode/.style={draw=black,fill=#1,minimum width=3mm,circle},
]

    \node[cnode=black,label=0:$y_2$] (sK) at (7,-4) {};
    \node[cnode=black,label=0:$y_1$] (s1) at (7,-2) {};
    \node[label=0:$\mathrm{outputs}$] at (7,-3) {};
    \node at (0,-3) {$\vdots$};
    \node at (2.5,-3) {$\vdots$};
    \node at (5,-3) {$\vdots$};

    % \foreach \x in {1,...,3}
    % {   \pgfmathparse{\x<3 ? \x : "D"} 
    % %\node[cnode=<colour>,label=<position in degrees of label>:<label text>] (<node reference for paths>) at (<x coord>, <y coord>){};
    %     \node[cnode=blue,label=180:$x_{\pgfmathresult}$] (x-\x) at (0,{-\x/0.75)}) {};
    %     \pgfmathparse{\x<3 ? \x : "N"} % Change result to print N for hidden layer
    %     \node[cnode=gray,label=90:$z_{1\pgfmathresult}$] (p-\x) at (3,{-\x/0.75)}) {};
    %     \pgfmathparse{\x<3 ? \x : "M"} % Change result to print M for hidden layer
    %     \node[cnode=gray,label=90:$z_{2\pgfmathresult}$] (p-\x) at (5,{-\x/0.75)}) {};
    %  % draw line from (here) -- <with label above> {<name>} (<to here>)        
    %     \draw (p-\x) -- node[above,sloped,pos=0.3] {${\scriptstyle w^{(3)}_{1\pgfmathresult}}$} (s1);
    % } % Bracket for loop
    

    \foreach \x in {1,...,3}
    {   \pgfmathparse{\x<3 ? \x : "D"} 
    %\node[cnode=<colour>,label=<position in degrees of label>:<label text>] (<node reference for paths>) at (<x coord>, <y coord>){};
        \node[cnode=blue,label=180:$x_{\pgfmathresult}$] (x-\x) at (0,{-\x/0.75)}) {};
        \pgfmathparse{\x<3 ? \x : "L"} % Change result to print N for hidden layer
        \node[cnode=gray,label=90:$z^{(1)}_{\pgfmathresult}$] (z-\x) at (2.5,{-\x/0.75)}) {};


        \pgfmathparse{\x<3 ? \x : "M"} % Change result to print M for hidden layer
        \node[cnode=gray,label=90:$z^{(2)}_{\pgfmathresult}$] (p-\x) at (5,{-\x/0.75)}) {};
        \draw (p-\x) -- node[above,sloped,pos=0.3] {${\scriptstyle w^{(3)}_{1\pgfmathresult}}$} (s1);

    } % Bracket for loop



    \foreach \x in {1,...,3}
    {   \foreach \y in {1}
        {   
    \pgfmathparse{\x<3 ? \x : "D"}        
        \draw (x-\x) --  node[above,sloped,pos=0.3] {$ {\scriptstyle w^{(1)}_{1\pgfmathresult}}$} (z-\y);
        }
    }


    \foreach \x in {1,...,3}
    {   \foreach \y in {1}
        {   
    \pgfmathparse{\x<3 ? \x : "L"}        
        \draw (z-\x) --  node[above,sloped,pos=0.3] {$ {\scriptstyle w^{(2)}_{1\pgfmathresult}}$} (p-\y);
        }
    }
\end{tikzpicture}
\end{center}
\caption{MLP architecture. For clarity the diagram displays connections for a few units. Each layer is fully connected with ReLU activations. Input dimensions $D = h_1 \times w_1 $. Number of hidden units in the first and second layers labelled $L$ and $M$ respectively.}
\label{fig:NN}

\end{figure}
